Feasibility of Non-Line-of-Sight Integrated Sensing and Communication at mmWave

One rarely addressed direction in the context of Integrated Sensing and Communication (ISAC) is non-line-of-sight (NLOS) sensing, with the potential to enable use cases like intrusion detection and to increase the value that wireless networks can bring. However, ISAC networks impose challenges for sensing due to their communication-oriented design. For instance, time division duplex transmission creates spectral holes in time, resulting in spectral replicas in the radar image. To counteract this, we evaluate different channel state information processing strategies and discuss their tradeoffs. We further propose an ensemble of techniques to detect targets in NLOS conditions. Our approaches are validated with experiments using a millimeter wave ISAC proof of concept in a factory-like environment. The results show that target detection in NLOS is generally possible with ISAC.

==> CutContent/discarded_1/Introduction.tex <==
\glsresetall

\section{Introduction}\label{sec:intro}

One of the key motivations behind the realization of the \gls{6G} of mobile networks is to augment networks with the ability to gather information about the surrounding environment.
The combination of this functionality with the existing cellular communication capabilities is referred to as \gls{isac}.
Compared to active localization in 5G (and earlier generations), where only active \glspl{ue} can be localized, \gls{isac} networks will be able to acquire information also from passive targets. The concept of \gls{ofdm} radar can be exploited for extracting information about range and relative speed of illuminated targets from the reflected radio signal.

Current research has been focusing, among other aspects, on the definition of plausible use cases of ISAC systems and their requirements. Applications range from vehicle sensing (automotive or aerial) to human activities detections and industrial floor monitoring~\cite{Mandelli_Henninger_Bauhofer_Wild_2023}.
The typical assumption is that targets will lie in \gls{los} from the sensing system.
However, especially for urban or indoor scenarios, this assumption often does not hold true, as the radio signal could reach targets not via the \gls{los} path but only after (multiple) reflections.
\newline \Gls{nlos} sensing in ISAC is still a rather unexplored area of research.
The primary benefit of \gls{nlos} sensing is the ability to perform 'around the corner' detection, which is not possible with traditional fixed camera or LIDAR systems. 
This feature would be particularly useful in applications such as automotive radar and surveillance systems, where it is necessary to detect targets moving behind obstacles.
Communication hardware operating in mmWave is expected to be deployed in indoor areas and factory floors. Intrusion detection in \gls{nlos} could represent a possible use case and a strong feature for private cellular networks in smart industries.
This work is intended as an initial exploration of the feasibility of monostatic \gls{nlos} sensing, focusing on intrusion detection scenarios in industrial environments.

The proposed approaches are validated using real-world measurements obtained from Nokia's ISAC mmWave prototype, deployed in the ARENA 2036 indoor industrial test facility in Stuttgart, Germany.


==> CutContent/discarded_1/Results.tex <==
%-----------------------------------------------------------------------------
% MEASUREMENTS
%-----------------------------------------------------------------------------
\section{Measurement Results}
\label{sec:meas_result}

%\subsection{Human Detection}

We tested the \gls{nlos} detection capabilities on human targets, moving in the ``emulated'' \gls{nlos} environment between wall and \gls{gnb} shown in Fig.~\ref{fig:nlos-meas_scheme_lateral}.
The results are compared for different values of processed frames $K$ after decimating the \glspl{csi} with decimation factors $J$, as presented in~\ref{sec:csi_strategies}.
The values for $K$ were chosen in a way to guarantee high enough SNR, while being able to generate at least 10 updates per second.
% Clutter removal was performed to ensure precise estimation of the expected target position in \gls{nlos} conditions, by using the methods presented in~\cite{Henninger_CRAP_2023}.
\todo[inline]{MH: previous sentence is a bit redundant imo, suggest to cut (or remove) it
\newline PT: I commented it out}
% CRAP has showed to outperform ECA-C in previously investigated \gls{los} scenarios due to its ability to isolate static targets and better separate them~\cite{Henninger_CRAP_2023}. 
% In NLOS ECA-C showed to enhance target returns, while the information about static targets would be discarded regardless.
%The detection rate was obtained by using CRAP for the \gls{los} region, while the \gls{nlos} peak detection was performed with ECA-C.
After computing the periodogram, targets were detected using the range-adjusted exponential threshold from Eq.~\eqref{eq:ra_cfar_thresh}.

%\paragraph{Results with CRAP:}
%\todo[inline]{SM: Actually, here there is a bit of miscommunications. You just finished saying that ECA-C does not work in NLOS and then you have two sections with CRAP vs. ECA-C, where - at a first glance - ECA-C performs better than CRAP. I think you need to better communicate that ECA-C is only applied for NLOS, while CRAP is still the logic for the LOS region and to rephrase all statements accordingly. My proposal would be to first state that CRAP has showed to outperform ECA-C in previously investigated LOS scenarios due to its ability to isolate static targets and better separate them. Then, in NLOS we tested both options bla bla...}

%\begin{table}[H]
%    % \caption*{\textbf{Example of Table}}
%    \centering 
%    \setlength{\abovecaptionskip}{5pt} % Adjust the space above the caption
%    \setlength{\belowcaptionskip}{0cm} % Adjust the space below the caption
%    \setlength{\intextsep}{1pt} % Adjust the space between the figure and the text
%    
%    \small
%    \begin{tabular}{| c | c | c |}
%    \hline
%    \rowcolor{bluePoli!40}
%    
%    $K$ & $J$  & \textbf{Detection rate}\T\B \\
%    \hline \hline
%    \footnotesize 1 & 1  & 0.26 \T\B \\ \hline
%    \footnotesize 1 & 47  & 0.15 \T\B \\ \hline
%    \footnotesize 6 & 70  & 0.37 \T\B \\ \hline
%    \footnotesize 10 & 70  & 0.54 \T\B \\ \hline
%    
%    \end{tabular}
%    \\[1pt]
%    \caption{\small Detection rate of a human target in \gls{nlos} evaluated after clutter removal with CRAP, peak detection with range-adjusted exponential threshold. $K$ and $J$ refer to number of processed frames, and symbol resampling interval, as defined in Section \ref{sec:csi_strategies}.}
%    \label{table:results_CRAP}
%\end{table}



\paragraph{Measured detection rate}

% CRAP and ECA-C were applied separately for the \gls{los} and \gls{nlos} region of the periodogram, respectively. 
Detection rate was estimated for the 10 strongest returns in \gls{nlos}, comparing them with the \gls{los} component.
%\todo[inline]{MH: what is $n$ here? If it's just a fixed number, just name it, no need to introduce a variable then (plus, $n$ is already used in the periodogram)
%\newline PT: changed $n$ to 10}

%Results presented in Table \ref{table:results_ECAC} show that ECA-C is able to enhance the performance of the system when compared to CRAP for \gls{nlos} components.
The measured detection rates for various \gls{csi} decimation strategies are shown in Table \ref{table:results_ECAC}.

\todo[inline]{MH: you should at least spend one sentence to comment on the results in the table. Btw, we don't have results for other configurations, right?}

\begin{table}[t]
     \caption{Measured detection rate.}\label{table:results_ECAC}
    % \caption*{\textbf{Example of Table}}
    \centering 
    \setlength{\abovecaptionskip}{5pt} % Adjust the space above the caption
    \setlength{\belowcaptionskip}{0cm} % Adjust the space below the caption
    \setlength{\intextsep}{1pt} % Adjust the space between the figure and the text
    
    \begin{tabu}{| c | c | c |}
    \hline
    Frames $K$ & Decimation $J$  & \textbf{Detection rate} \\
    \Xhline{3\arrayrulewidth}
     4 & 70  & 0.61  \\ \hline
     6 & 70  & 0.60  \\ \hline
     8 & 70  & 0.67  \\ \hline

    \end{tabu}
\end{table}

\paragraph{Detection moving average}

With the focus on intrusion detection, it is sufficient to detect the presence of the intruder once and raise an alarm accordingly.
A possible approach for discriminating the presence of actual targets from false alarms is to verify that \gls{nlos} peaks are continuously detected within a window of consecutive updates.
The sustained presence of the \gls{nlos} return over an observation window can be evaluated by computing the moving average of the detection rate over time. Fig.~\ref{fig:detect_mov_avg} depicts the detection rate evaluated over a 0.5~s time window across the measured scenario.
\todo[inline]{MH: what is the configuration you were using for the result in Fig. 5?
\newline PT: 8 frames, with frame stride of 2}
\begin{figure}[t]
    \setlength{\abovecaptionskip}{3pt} % Adjust the space above the caption
    \setlength{\belowcaptionskip}{3pt} % Adjust the space below the caption
    \setlength{\intextsep}{4pt} % Adjust the space between the figure and the text
    \centering
    \includegraphics[width=0.95\columnwidth, height = 5.5cm]{Images/detect_mov_avg_bluepoli_highlighted.png}
    \caption{Moving average of NLOS detections over a 0.5 s time window, using exponential threshold and clutter removal. Periodograms were generating using CSI matrices from $K=8$ frames.
    % The red and blue dashed lines highlight the target stopping to change direction and moving in the test area of Section \ref{sec:meas_setup}, respectively. 
    }
    \label{fig:detect_mov_avg}
\end{figure}

The calculation of the detection rate includes the parts of the measurements where the target stopped and changed direction (highlighted in red in Fig.~\ref{fig:detect_mov_avg}).
In these instances detection is negative, since no \gls{nlos} component is detected, as the bins of the periodogram corresponding to zero speed are discarded as described in~\ref{subsec:NLOS_processing}.


==> CutContent/discarded_1/System.tex <==
\section{Measurement Setup}\label{sec:PoCScenario}

%\todo[inline]{PT: Remove repetition}

%Before describing the proposed \gls{nlos} detection approach in Section~\ref{sec:equations_and_figures}, a brief introduction to the \gls{isac} \gls{poc} and the \gls{nlos} measurement scenario are given in the following.

\subsection{ISAC PoC}
This work was developed based on real-world measurement data obtained from an \gls{isac} \gls{poc}, based on commercially
available \gls{5G} communications hardware in \gls{fr2}.
The system comprises a mmWave \gls{gnb} \gls{ru} acting as TX, extended by a dedicated sniffer \gls{ru} serving as RX, as well as a server called \gls{spu}. The radios are physically separated, but quasi co-located, allowing to treat the system as a mono-static sensing setup. The \gls{gnb} transmits a \gls{5G} \gls{ofdm} signal in \gls{tdd} mode.
The sniffer is synchronized with the \gls{gnb} and always operates in \gls{ul} mode. 
%After FFT and \gls{cp} removal, 
The \gls{spu} receives the complex IQ signal and computes the \gls{csi} matrix $\mathbf H \in \mathbb{C}^{N\times M}$ via division of the reflected signal by the transmitted signal per radio frame ($10$~ms duration), which serves as input for sensing processing. The operating parameters of the prototype based on numerology $\mu = 3$~\cite{3gpp_38211} are listed in Tab.~~\ref{table:PoC_params}. For more details, please refer to~\cite{Wild_Grudnitsky_Mandelli_Henninger_Guan_Schaich_2023}. 

%------------------------------------------------------------------------------------------------------------------------------------
\subsection{Ideal System Performance}

%\todo[inline]{MH: here we assume some knowledge of \gls{ofdm} radar already, but we probably don't have space to introduce it anyway}

\begin{table}[t]
    \caption{POC System parameters.}\label{table:PoC_params}
	\centering
     \begin{tabu}{|l|l|r|}
            \hline
            \textbf{Parameter} & \textbf{Description} & \textbf{Value} \\
			\Xhline{3\arrayrulewidth}
			$f_c$ & Carrier frequency & 27.4 GHz \\
  			\hline
            $B$ & Total bandwidth $N\cdot \Delta f$ & 190 MHz \\
  			\hline
  			$N$ & Number of subcarriers & 1584 \\
            \hline
  			$M$ & Number of \gls{ofdm} symbols per radio frame & 1120\\
  			\hline
  			$\Delta f$ & Subcarrier spacing & 120 kHz\\
  			\hline
  			$T_0$ & OFDM symbol time & 8.33 $\upmu$s\\
            \hline
            $T_{\text{CP}}$ & CP length & 0.59 $\upmu$s \\
  			\hline
  			$T_{s}$ & OFDM symbol time including CP & 8.92 $\upmu$s \\
  			\hline
    \end{tabu}
\end{table}

The achievable system performance can be evaluated in terms of resolution and unambiguous aperture, for both range and speed.
Unambiguous range $d_{\text{unamb}}$ and speed $v_{\text{unamb}}$ are the maximum values without ambiguities due to aliasing, and depend on the sampling rate in frequency and time domain, defined by the subcarrier spacing $\Delta f$ and the \gls{ofdm} symbol time $T_s$, respectively. Range and speed resolution, $d_{\text{res}}$ and $v_{\text{res}}$, refer to the ability to discriminate targets based on their range and speed. The resolution depends on the aperture in frequency and time, given by the bandwidth $N\cdot\Delta f$ and the frame duration $M \cdot T_S$, respectively. 
Computing the periodogram by processing the \gls{csi} of a single frame with the parameters from Tab.~\ref{table:PoC_params},
the performance of the \gls{poc} can be derived as in~\cite{Nuss_Mayer_Performance} and is presented in Tab.~\ref{table:PoC_performance}.
\begin{table}[t]
    \caption{POC Ideal performance.}\label{table:PoC_performance}
	\centering
     \begin{tabu}{|l|l|l|}
            \hline
            \textbf{Parameter} & \textbf{Description} & \textbf{Value} \\
			\Xhline{3\arrayrulewidth}
			$v_{\text{unamb}}$ & Unambiguous speed & 613.5~\text{m/s} \\
  			\hline
            $d_{\text{unamb}}$ & Unambiguous range & 1250~\text{m} \\
  			\hline
  			$v_{\text{res}}$ & Speed resolution & 0.565 \text{ m/s} \\
            \hline
  			$d_{\text{res}}$ & Range resolution & 0.789~\text{m}\\
  			\hline
    \end{tabu}
\end{table}
\todo[inline]{MH: fix speed resolution}
An additional parameter to consider is the \gls{snr} in the periodogram, which scales linearly with the number of elements in $\mathbf H$ used for sensing.
A high \gls{snr} is essential to distinguish peaks from the underlying noise floor. This is especially critical for \gls{nlos} measurements, where the received reflected signal power is typically low due to the propagation distance and multiple reflections.

\subsection{NLOS Scenario}
\label{sec:meas_setup}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{Images/meas_scheme/Base-lateral_view_update2.png}
    \caption{\small Geometry of the measurement scenario. The target moves back and forth in a straight line between the wall and the \gls{gnb}.}
    \label{fig:nlos-meas_scheme_lateral}
\end{figure}

\todo[inline]{MH: actually a photo of the investigation would be nice in addition to the sketch in Fig. 1., but probably we don't have enough space}

The two \glspl{ru} of the \gls{isac} \gls{poc} are mounted at a height of $h_{\text{gNB}} = 5.12$~m and oriented towards a wide investigation area in the ARENA2036 industrial research campus in Stuttgart, Germany. The antenna pole is located at a horizontal distance of approximately $d_{\text{wall}}=23$~m from a warehouse rack (installed in front of a concrete wall) and a cargo door.
The measurement area is free of major obstructions that could be used to create a \gls{nlos} scenario under normal conditions. 
However, it is possible to emulate \gls{nlos} conditions by directing the signal over the target towards the wall and observing the reflected returns, as shown in Fig.~\ref{fig:nlos-meas_scheme_lateral}. Further, due to the large beamwidth, both \gls{los} and \gls{nlos} returns are present in our measurements. The \gls{los} component is critical for our study as it represents a source of ground truth and can be used as a rough estimate of the target position. Note, however, that this information has no bearing on the \gls{nlos} detection capabilities of our setup, but it is merely used as a simple remedy in the absence of accurate ground truth information.

%\subsection*{Detection rate}
The scope of the experiments with the described setup was to determine the presence of the target via the \gls{nlos} return. 
At each update, given the geometry of the measurement described in Fig.~\ref{fig:nlos-meas_scheme_lateral}, the expected speed and range of the target is estimated from the \gls{los} position as
\todo[inline]{MH: commented out the commands that squish the equations, let's use them only as last resport}
%\setlength{\abovedisplayskip}{3pt}
%\setlength{\belowdisplayskip}{3pt}
\begin{align}
    \hat{v}_{\text{NLOS}} &\approx -v_{\text{LOS}} \; ,  \\
    \hat{d}_{\text{NLOS}} &= 2 d_{\text{wall}} - d_{\text{LOS}}\cdot \sin{\left(\theta_{\text{LOS}}\right)} \; ,
\end{align}
where $\theta_{\text{LOS}} = \arccos{\left(h_{\text{gNB}}/d_{\text{LOS}}\right)}$.
%\[
%\begin{array}{ll}
%    &\hat{v}_{\text{NLOS}} = -v_{\text{LOS}},   \\
 %   &\hat{d}_{\text{NLOS}} = 2 d_{\text{wall}} - d_{\text{LOS}}\cdot \cos{\left(\arctan{\left(\frac{h_{\text{gNB}}}{d_{\text{LOS}}}\right)}\right)}.
%\end{array}
%\]
%\end{aligned}
%\end{cases}
%\end{equation*}
%\todo[inline]{MH: here you mention NLOS region already, but you have not introduced it yet, right?}
Peaks detected in the \gls{nlos} region are compared with the expected target position, allowing to determine whether they correspond to the return generated by the moving actor or to interference.
If the measured \gls{nlos} range and speed match those estimated from ground truth, detection is positive.
The detection rate is computed as the ratio of frames in which the \gls{nlos} component was detected to the total number of frames in which the \gls{los} component was detected.

==> CutContent/discarded_1/System_old.tex <==
%----------------------------------------------------------------------------
% SYSTEM MODEL
%-----------------------------------------------------------------------------

\section{System Model and PoC Setup}\label{sec:system_model}

\gls{ofdm} radio signals, which are transmitted by base stations to users and vice versa, not only carry data but are also affected by the movement of the transmitter, obstacles, and illuminated targets.
The system consists of physically separated TX and RX.
The TX operates at center frequency $f_C$, transmitting $M$ OFDM symbols over $N$ subcarriers spaced by $\Delta f$, carrying complex modulation symbols.
The entirety of the $N \times M$ transmitted symbols are referred to as OFDM frame $\mathbf F_{Tx} \in \mathbbm{C}^{N\times M}$.
The transmitted signal is reflected by passive targets in the environment.
For a scenario where the beam illuminates $H$ targets, each one is indexed as $h \in H$ and its influence on the signal depends on its range $d_h$ and its speed $v_h$ relative to the RX.
The received OFDM frame is $\mathbf F_{Rx} \in \mathbbm{C}^{N\text{x}M}$, which can be expressed as the superposition of the reflected paths generated from reflection of the signal upon the $H$ targets.
The \gls{csi} can be obtained by dividing the received frame with the known transmitted one \cite{Braun2014OFDMRA}.
After element-wise division the \gls{csi} is
\begin{equation*}
    \mathbf F = e^{j\phi} \cdot \sum_{h\in H} b_h \mathbf a(d_h) \mathbf b(v_h)^T + \mathbf{Z},
\end{equation*}
where $b_h$ is the complex coefficient related to the \textit{h}-th reflector, $\phi$ is a random phase term to model phase incoherence between different acquisitions, and
$\mathbf Z \in \mathbbm{C}^{N\times M}$ indicates the random complex \gls{awgn} matrix. Further, the vectors
describing the linear phase shifts over subcarriers and symbols due to range $d_h$ and $v_h$, respectively, write as
\begin{align*}
    \bm{a}(d_h) &= \left[1, e^{-j4\pi \Delta f \cdot d_h / c}, ..., e^{-j4\pi(N-1)\Delta f \cdot d_h / c} \right]^\text T \\
    \bm{b}(v_h) &= \left[ 1, e^{j4\pi T_s f_c \cdot v_h / c}, ..., e^{j4\pi (M-1) T_s f_c \cdot v_h / c} \right]^\text{T}
\end{align*}
with $c$ denoting the speed of light and $T_s$ the \gls{ofdm} symbol time including \gls{cp}.
%Vectors $\bm a(d_h)$ and $\bm b(v_h)$ represent information about target's range $d_h$ and speed $v_h$, encoded on the reflected signal's frequency and time domain, respectively.
Range and speed of the targets can be estimated from the \gls{csi}, \egc through spectral estimation methods.
These can be divided in non-parametric (\egc periodogram) and parametric methods (\egc MUSIC, ESPRIT).
This work will focus on spectral estimation with periodogram due to its computational efficiency compared to parametric methods.
The 2D periodogram is obtained by computing one DFT for each OFDM symbol, followed by $N$ iDFTs, one for each subcarrier of $\mathbf F$ as
\begin{equation}
\begin{split}
S(n,m) &= \frac{1}{N'M'}\left|\sum_{k=0}^{N'} \Biggl(\sum_{l=0}^{M'} \mathbf{F}(k, l)e^{-j2\pi\frac{lm}{M'}}\Biggr)e^{j2\pi\frac{kn}{N'}} \right|^2, \\[-2ex]
\end{split}
\label{eq:periodogram}
\end{equation}
where $N' = 2^{\ceil{\log_2{N}}}$ and $M' = 2^{\ceil{\log_2{M}}}$ are the number of rows and columns of $\mathbf{F}$ after zero padding. 

\subsection{Nokia's ISAC FR2 Prototype}

The described system model can be linked to Nokia's ISAC \gls{poc}, based on \gls{fr2} 5G commercially available communication hardware \cite{Wild_Grudnitsky_Mandelli_Henninger_Guan_Schaich_2023}. Operating parameters for the prototype are listed in Table \ref{table:PoC_params}.
The system comprises a mmWave \gls{gnb} \gls{ru}, extended by a dedicated \textit{Sniffer} \gls{ru} and a server called \gls{spu}.
The \gls{gnb} operates in Time Division Duplexing (TDD) mode.
The sniffer is synchronized with the \gls{gnb} by the same synchronization source and it always operates in \gls{ul} mode. 
The \gls{spu} receives the complex IQ signal, after FFT and removal of the \gls{cp}, as input for the sensing processing on a per-radio frame basis.

%------------------------------------------------------------------------------------------------------------------------------------
\subsection{Ideal System Performance}
\begin{table}[b]
    % \caption*{\textbf{Example of Table}}
    \centering 
    \small
    \begin{tabular}{|c | c | c |}
    \hline
    %\rowcolor{bluePoli!40}
    \textbf{Parameter} & \textbf{Description} & \textbf{Value} \T\B \\
    \hline \hline
    $f_c$ & \small carrier frequency & 27.4 GHz \T\B \\ \hline
    $N$ & \small subcarriers & 1584  \T\B \\ \hline
    $M$ & \small OFDM symbols & 1120  \T\B\\ \hline
    $\Delta f$ & \small subcarrier spacing & 120 kHz  \T\B\\ \hline
    $T_0$ & \small OFDM symbol time & 8.33 $\mu$s  \T\B\\ \hline
    $T_{CP}$ & \small CP interval & 0.59 $\mu$s  \T\B\\ \hline
    $T_{s}$ & \small symbol time incl. CP & 8.92 $\mu$s  \T\B\\ 
    \hline
    \end{tabular}
    \\[1pt]
    \caption{System parameters considered for Nokia's PoC.}
    \label{table:PoC_params}
\end{table}

System performance can be evaluated in terms of resolution and unambiguous aperture, for both range and speed.
Unambiguous range $d_{\text{unamb}}$ and speed $v_{\text{unamb}}$ are the maximum values that can be measured for a target without any ambiguity or ambiguity-related errors, and depend on the sampling rate in the respective domain, defined by subcarrier spacing and OFDM symbol time, respectively.
Range and speed resolution, $d_{\text{res}}$ and $v_{\text{res}}$, refer to the system's ability to resolve targets in terms of their range and speed and depend on the aperture in frequency and time domain, given by the overall bandwidth $\Delta f N$ and the frame duration $T_S M$, respectively. 
When generating the periodogram by processing the CSI of a single frame, with the parameters indicated in Table \ref{table:PoC_params},
the \gls{poc} operates with the following performance
%\begin{equation*}
%\begin{cases}
%    &v_{\text{unamb}} = \frac{c_0}{2f_C T_S} = 613.5\text{ m/s} \:,  \\
%    &d_{\text{unamb}} = \frac{c_0}{2\Delta f} = 1250 \text{ m} \:, \\
%    &v_{\text{res}} = \frac{c_0}{2T_Sf_CM} = 0.547 \text{ m/s} \:, \\
%    &d_{\text{res}} = \frac{c_0}{2\Delta fN} = 0.789 \text{ m} \; . \\   
%\end{cases}
%\end{equation*}

\[
\renewcommand{\arraystretch}{1.5}
\begin{array}{ll}
v_{\text{unamb}} = \frac{c_0}{2f_C T_S} = 613.5\text{ m/s} & , \\
d_{\text{unamb}} = \frac{c_0}{2\Delta f} = 1250 \text{ m} & , \\
v_{\text{res}} = \frac{c_0}{2T_Sf_CM} = 0.547 \text{ m/s} & , \\
d_{\text{res}} = \frac{c_0}{2\Delta fN} = 0.789 \text{ m} & . \\
\end{array}
\]

An additional parameter to consider is the \gls{snr} in the periodogram, which scales linearly with the number of elements in the \gls{csi} used for sensing.
A high \gls{snr} is essential to distinguish peaks from the underlying noise floor, especially for \gls{nlos} measurements where the received reflected signal power is typically low due to the propagation distance and multiple reflections.

\subsection{Measurement Principle and Scenario}
\label{sec:meas_setup}

Nokia's ISAC prototype was mounted in an indoor industrial test facility, with gNB and sniffer positioned at a height of $5.12$ m. The transmitter was oriented towards a wide  indoor area free of obstacles. The antenna pole was located approximately 23 m from a warehouse rack (installed in front of a concrete wall) and a cargo door.
The observed measurement area was free of any major obstructions or occlusions that could be used to create a \gls{nlos} scenario under normal conditions. 
Nonetheless, it was possible to generate \gls{nlos} conditions by directing the signal over the target and towards the wall, observing the reflected returns.
Due to the large beamwidth, both \gls{los} and \gls{nlos} components can be jointly observed in our measurements, as shown in Figure~\ref{fig:nlos-meas_scheme_lateral}.

The observed \gls{los} component is critical for our study since it represents a source of ground truth and can be used as a correct estimate of the position of the target in the test area. Note that this information has no bearing on the \gls{nlos} detection capabilities of our setup, but it is merely used as a simple remedy in the absence of accurate ground truth information.
\begin{figure}[b]
    \centering
    \includegraphics[width=0.42\textwidth]{Images/base-lateral_view_los_geometry_noaxis.png}
    \caption{\small Geometry of the measurement. Target moves between wall and \gls{gnb} and back in a straight line.}
    \label{fig:nlos-meas_scheme_lateral}
\end{figure}

%\subsection*{Detection rate}
The scope of the measurement was to determine the presence and the characteristics of the \gls{nlos} return. 
At each target update, given the geometry of the measurement described in Figure \ref{fig:nlos-meas_scheme_lateral}, the expected range and speed of the target was estimated from the \gls{los} position as
%\begin{equation*}
%\begin{cases}
%\begin{aligned}
\[
\begin{array}{ll}
    &\hat{v}_{\text{NLOS}} = -v_{\text{LOS}},   \\
    &\hat{d}_{\text{NLOS}} = 2 d_{\text{wall}} - d_{\text{LOS}}\cdot \cos{\left(\arctan{\left(\frac{h_{\text{gNB}}}{d_{\text{LOS}}}\right)}\right)}.
\end{array}
\]
%\end{aligned}
%\end{cases}
%\end{equation*}

Peaks detected in the \gls{nlos} region were compared with the expected target position, allowing to determine if they correspond to the return generated by the moving actor or to interference.
If the measured \gls{nlos} range and speed corresponded to the one estimated from ground truth, detection was positive.
The detection rate was calculated as the ratio of frames in which the \gls{nlos} component was detected to the total number of frames in which the \gls{los} component was detected.


==> CutContent/discarded_2/System.tex <==
\section{ISAC Setup}\label{sec:PoCScenario}

%\todo[inline]{PT: Remove repetition}

%Before describing the proposed \gls{nlos} detection approach in Section~\ref{sec:equations_and_figures}, a brief introduction to the \gls{isac} \gls{poc} and the \gls{nlos} measurement scenario are given in the following.

\subsection{ISAC PoC}
This work was developed based on real-world measurement data obtained from our \gls{isac} \gls{poc}~\cite{wild2023integrated}, based on commercially
available \gls{5G} communications hardware in \gls{fr2} at central frequency $f_c = 27.4$~GHz.
The system comprises a half-duplex \gls{gnb} \gls{ru} acting as \gls{tx}, extended by a dedicated sniffer \gls{ru} serving as \gls{rx}.
%, as well as a server called \gls{spu}.
\todo[inline]{SM: define TX/RX as acronyms. Then, use either ``radio'' or ``gNB'' (I would go for radios, to be honest), or - better - RU everywhere}
The radios are physically separated, but quasi co-located, allowing to treat the system as a mono-static sensing setup. The \gls{gnb} transmits a \gls{5G} \gls{ofdm} signal in \gls{tdd} mode (4:1 \gls{dl}/\gls{ul} ratio).
\todo[inline]{SM: introduce the 4:1 split here}
The sniffer is synchronized with the \gls{gnb} by fiber connection to a common sync source and always operates in \gls{ul} mode. 
\todo[inline]{SM: can we say how it is synchronized? If not, it's not important (``via direct cable connection'' would also be sufficient)
\newline PT: added connection to common sync source}
%After FFT and \gls{cp} removal, 
A dedicated server receives the complex IQ signal and computes the \gls{csi} matrix $\mathbf H \in \mathbb{C}^{N\times M}$ via division of the reflected signal by the transmitted signal per radio frame ($10$~ms duration).
%, which serves as input for sensing processing. 
The operating parameters of the prototype based on \gls{3GPP} numerology $\mu = 3$~\cite{3gpp_38211} are listed in Tab.~~\ref{table:PoC_params}. For more details, please refer to~\cite{wild2023integrated}. 

%------------------------------------------------------------------------------------------------------------------------------------
\subsection{Ideal System Performance}

%\todo[inline]{MH: here we assume some knowledge of \gls{ofdm} radar already, but we probably don't have space to introduce it anyway}

\begin{table}[t]
    \caption{POC System parameters.}\label{table:PoC_params}
	\centering
     \begin{tabu}{|l|l|r|}
            \hline
            \textbf{Parameter} & \textbf{Description} & \textbf{Value} \\
			\Xhline{3\arrayrulewidth}
			$f_c$ & Carrier frequency & 27.4 GHz \\
  			\hline
            $B$ & Total bandwidth $N\cdot \Delta f$ & 190 MHz \\
  			\hline
  			$N$ & Number of subcarriers & 1584 \\
            \hline
  			$M$ & Number of \gls{ofdm} symbols per radio frame & 1120\\
  			\hline
  			$\Delta f$ & Subcarrier spacing & 120 kHz\\
  			\hline
  			$T_0$ & OFDM symbol time & 8.33 $\upmu$s\\
            \hline
            $T_{\text{CP}}$ & CP length & 0.59 $\upmu$s \\
  			\hline
  			$T_{s}$ & OFDM symbol time including CP & 8.92 $\upmu$s \\
  			\hline
    \end{tabu}
\end{table}

The achievable system performance can be evaluated in terms of resolution and unambiguous aperture, for both range and speed.
\todo[inline]{SM: should we mention somewhere that - for simplicity - we focus our analysis on the acquisitions given by a single beam, corresponding to a X deg main lobe bla bla?}
Unambiguous range $d_{\text{unamb}}$ and speed $v_{\text{unamb}}$ are the maximum values without ambiguities due to aliasing, and depend on the sampling rate in frequency and time domain, defined by the subcarrier spacing $\Delta f$ and the \gls{ofdm} symbol time $T_s$, respectively. Range and speed resolution, $d_{\text{res}}$ and $v_{\text{res}}$, refer to the ability to discriminate targets based on their range and speed. The resolution depends on the aperture in frequency and time, given by the bandwidth $N\Delta f$ and the frame duration $M T_S$, respectively. 
\todo[inline]{SM: add one radar reference here, you can use Lucas'. Btw, I would also add the reference just after ``periodogram''.

Moreover, not sure whether the cdot is required in the expressions above}
Computing the periodogram by processing the \gls{csi} of a single frame with the parameters from Tab.~\ref{table:PoC_params},
the \gls{poc} operates with the following performance
\begin{align}
v_{\text{unamb}} &= \frac{c_0}{2f_C T_s} = 613.5~\text{m/s} \; , \label{eq:speed_unamb} \\
d_{\text{unamb}} &= \frac{c_0}{2\Delta f} = 1250~\text{m} \; , \\
v_{\text{res}} &= \frac{c_0}{2T_sf_CM} = 0.547 \text{ m/s} \; , \label{eq:speed_res} \\
d_{\text{res}} &= \frac{c_0}{2\Delta fN} = 0.789~\text{m} \; .
\end{align}
%\[
%\renewcommand{\arraystretch}{1.5}
%\begin{array}{ll}
%v_{\text{unamb}} = \frac{c_0}{2f_C T_S} = %613.5\text{ m/s} & , \\
%d_{\text{unamb}} = \frac{c_0}{2\Delta f} = 1250 \text{ m} & , \\
%v_{\text{res}} = \frac{c_0}{2T_Sf_CM} = 0.547 \text{ m/s} & , \\
%d_{\text{res}} = \frac{c_0}{2\Delta fN} = 0.789 \text{ m} & . \\
%\end{array}
%\]
%\todo[inline]{MH: fix speed resolution}
An additional parameter to consider is the \gls{snr} in the periodogram, which scales linearly with the number of elements in $\mathbf H$ used for sensing.
\todo[inline]{SM: the previous sentence should be better explained, since it's not technically sound}
A high \gls{snr} is essential to distinguish peaks from the underlying noise floor. This is especially critical for \gls{nlos} measurements, where the received reflected signal power is typically low due to the propagation distance and multiple reflections.

\subsection{NLOS Scenario}
\label{sec:meas_setup}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{Images/meas_scheme/Base-lateral_view_final1.pdf}
    \caption{\small Geometry of the measurement scenario. The target moves back and forth in a straight line between the wall and the \gls{gnb}.}
    \label{fig:nlos-meas_scheme_lateral}
\end{figure}

%\todo[inline]{MH: actually a photo of the investigation would be nice in addition to the sketch in Fig. 1., but probably we don't have enough space}

The two \glspl{ru} of the \gls{isac} \gls{poc} are mounted at a height of $h_{\text{gNB}} = 5.12$~m and oriented towards a wide investigation area in the ARENA2036 industrial research campus in Stuttgart, Germany. The antenna pole is located at a horizontal distance of approximately $d_{\text{wall}}=23$~m from a warehouse rack (installed in front of a concrete wall) and a cargo door.
The measurement area is free of major obstructions that could be used to create a \gls{nlos} scenario under normal conditions. 
However, it is possible to emulate \gls{nlos} conditions by directing the signal over the target towards the wall and observing the reflected returns, as shown in Fig.~\ref{fig:nlos-meas_scheme_lateral}. Further, due to the large beamwidth, both \gls{los} and \gls{nlos} returns are present in our measurements. The \gls{los} component is critical for our study as it represents a source of ground truth and can be used as a rough estimate of the target position. Note, however, that this information has no bearing on the \gls{nlos} detection capabilities of our setup, but it is merely used as a simple remedy in the absence of accurate ground truth information.

%\subsection*{Detection rate}
The scope of the experiments with the described setup was to determine the presence of the target via the \gls{nlos} return. 
At each update, given the geometry of the measurement described in Fig.~\ref{fig:nlos-meas_scheme_lateral}, the expected speed and range of the target is estimated from the \gls{los} position as
\todo[inline]{MH: commented out the commands that squish the equations, let's use them only as last resort}
%\setlength{\abovedisplayskip}{3pt}
%\setlength{\belowdisplayskip}{3pt}
\begin{align}
    \hat{v}_{\text{NLOS}} &\approx -v_{\text{LOS}} \; ,  \\
    \hat{d}_{\text{NLOS}} &= 2 d_{\text{wall}} - d_{\text{LOS}}\cdot \sin{\left(\theta_{\text{LOS}}\right)} \; ,
\end{align}
where $\theta_{\text{LOS}} = \arccos{\left(h_{\text{gNB}}/d_{\text{LOS}}\right)}$.
%\[
%\begin{array}{ll}
%    &\hat{v}_{\text{NLOS}} = -v_{\text{LOS}},   \\
 %   &\hat{d}_{\text{NLOS}} = 2 d_{\text{wall}} - d_{\text{LOS}}\cdot \cos{\left(\arctan{\left(\frac{h_{\text{gNB}}}{d_{\text{LOS}}}\right)}\right)}.
%\end{array}
%\]
%\end{aligned}
%\end{cases}
%\end{equation*}
%\todo[inline]{MH: here you mention NLOS region already, but you have not introduced it yet, right?}
Peaks detected in the \gls{nlos} region are compared with the expected target position, allowing to determine whether they correspond to the return generated by the moving actor or to interference.
If the measured \gls{nlos} range and speed match those estimated from ground truth, detection is positive.
The detection rate is computed as the ratio of frames in which the \gls{nlos} component was detected to the total number of frames in which the \gls{los} component was detected.
\todo[inline]{SM: to be honest, this (C) part should be moved after the spectral holes thingy, since (i) it's part of our contribution, (ii) from a logical standpoint it's a bit better in my opinion.
First we introduce the issues of spectral holes (always present), how to compensate them to improve SNR, and then finally how everything is applied in a NLOS scenario. Otherwise, you first say you need high SNR (end of II.B), then you introduce your scenario and some processing (II.C), but then you say it's impossible to do it due to holes (in this case, they are not ``spectral'' in the close meaning, I would call them ``Time-domain holes''), and then that you compensate for this issue. By the end of it, the reader might have forgotten your NLOS setup/scenario}
